Topological Characterization of Consensus in Distributed Systems

We provide a complete characterization of both uniform and non-uniform deterministic consensus solvability in distributed systems with benign process and communication faults using point-set topology. More specifically, we non-trivially extend the approach introduced by Alpern and Schneider in 1985, by introducing novel fault-aware topologies on the space of infinite executions: the process-view topology, induced by a distance function that relies on the local view of a given process in an execution, and the minimum topology, which is induced by a distance function that focuses on the local view of the process that is the last to distinguish two executions. Consensus is solvable in a given model if and only if the sets of admissible executions leading to different decision values is disconnected in these topologies. By applying our approach to a wide range of different applications, we provide a topological explanation of a number of existing algorithms and impossibility results and develop several new ones, including a general equivalence of the strong and weak validity conditions.

==> applications.tex <==
\section{Applications}
\label{sec:applications}

In this section, we will apply our various topological characterizations of consensus solvability to
particular classes of examples. We start in Section~\ref{sec:bivalence} with the broad 
class of message adversaries that have been shown, or can be shown, to
make consensus impossible by means of bivalence proofs. We the proceed with 
a complete characterization of consensus solvability
the class of compact message adversaries
in Section~\ref{sec:closed}. A characterization for 
the class of non-compact message adversaries will be provided in Section~\ref{sec:nonclosed}.


\todo{US: MA-related definitions from the PODC paper - need adaption.}


A {\em communication graph\/} is any directed graph $G = ([n],E), E\subseteq
[n]\times[n]$ with node set~$[n]$.
A {\em message adversary\/} (MA) is a set of infinite sequences of communication graphs.
Graph sequences in this set are called {\em admissible\/} under the message adversary.

An algorithm~$\A$, an initial configuration~$C^0$ of~$\A$,
and a graph sequence $\mathbf{G} = (G^t)_{t\geq 1}$ uniquely 
determine an {\em execution\/} 
in a round-by-round 
fashion: 
During round~$t$, every process~$p$ updates its previous local state~$C_p^{t-1}$
to its new state~$C_p^t$ in a 
deterministic way according to~$\A$, based on the messages it received during
round~$t$.
Rounds advance synchronously in a send--receive--compute order.
Messages in round~$t$ are delivered according to communication graph~$G^t$:
Process~$q$ receives process~$p$'s message in round~$t$ if and only if $(p,q)$
is an edge of~$G^t$. 

An algorithm is defined by the local transition function and a set of initial
states for every process.
Since we are only interested in consensus algorithms, we stipulate that
processes have an initial state for every initial value~$v$ of the finite input
domain~$\VI$. Note carefully that we assume that a process running $\A$ 
does not know $n$ a priori, and cannot always infer $n$ from the
messages it receives in an execution either. By contrast, the message adversary 
need not be oblivious w.r.t.\ the algorithm, i.e., it may know $\A$ and choose its graph 
sequences accordingly.

A {\em configuration\/} is a tuple $(C_1,\dots,C_n)$ of process states.
Whenever~$\A$ is clear from the context, we denote its set of possible
configurations by~$\C$.
$\Comega$ denotes the set of all infinite sequences of configurations,
$\Gamma\subseteq \Comega$ is the set of admissible executions
resulting from admissible graph sequences.
Executions are represented by Greek letters $\alpha, \beta, \dots$.

\section{Process-Time Graphs}\label{sec:pt}

We will consider
\emph{process-time graphs}~\cite{BM14:JACM}, which are useful
for reasoning about the \emph{causal past} of a process
in a given round, and 
which will play a crucial role in our topological framework. 

For every graph sequence $\mathbf{G} = (G^t)_{t\geq 1}$ and every assignment of
initial values $x\in \VI^n$ to the~$n$ processes, we inductively construct the
following sequence of process-time graphs $PT^t$:

\begin{itemize}
\item
The process-time graph~$PT^0$ at time~$0$ contains the nodes $(p,0,x_p)$ for all processes $p\in[n]$, with input value $x_p\in\VI$,
and no edges.

\item
The process-time graph~$PT^1$ at time~$1$ contains the nodes $(p,0,x_p)$ and $(p,1)$ for all processes $p\in[n]$.
It contains an edge from $(p,0,x_p)$ to $(q,1)$ if and only if $(p,q)\in G^1$.

\item
For $t\geq 2$, the process-time graph~$PT^t$ at time~$t$ contains the nodes of~$PT^{t-1}$
and the nodes $(p,t)$ for all processes $p\in[n]$.
It contains an edge from $(p,t-1)$ to $(q,t)$ if and only if $(p,q)\in G^t$.
\end{itemize}

Figure~\ref{fig:pt} contains an example of a process-time graph at time~$2$.

\begin{figure}
\begin{tikzpicture}[>=latex']
\node[black!30!green, very thick, draw, circle,label=left:{$(1,0,1)$}] (C10) at (-3, 0)  {};
\node[black!30!green, very thick, draw, circle,label=left:{$(2,0,0)$}] (C20) at ( 0, 0)  {};
\node[black!30!green, very thick, draw, circle,label=left:{$(3,0,1)$}] (C30) at ( 3, 0)  {};

\node[black!30!green, very thick, draw, circle,label=left:{$(1,1)$}] (C11) at (-3, 2)  {};
\node[black!30!green, very thick, draw, circle,label=left:{$(2,1)$}] (C21) at ( 0, 2)  {};
\node[draw, circle,            label=left:{$(3,1)$}] (C31) at ( 3, 2)  {};

\node[black!30!green, very thick, draw, circle,label=left:{$(1,2)$}] (C12) at (-3, 4)  {};
\node[draw, circle,            label=left:{$(2,2)$}] (C22) at ( 0, 4)  {};
\node[draw, circle,            label=left:{$(3,2)$}] (C32) at ( 3, 4)  {};

\draw[black!30!green, very thick,->] (C10) -- (C11);
\draw[black!30!green, very thick,->] (C20) -- (C21);
\draw[->] (C30) -- (C31);
\draw[black!30!green, very thick,->] (C20) -- (C11);
\draw[black!30!green, very thick,->] (C30) -- (C21);
\draw[black!30!green, very thick,->] (C10) -- (C21);
\draw[->] (C20) -- (C31);

\draw[black!30!green, very thick,->] (C11) -- (C12);
\draw[->] (C21) -- (C22);
\draw[->] (C31) -- (C32);
\draw[black!30!green, very thick,->] (C21) -- (C12);
\draw[->] (C31) -- (C22);
\draw[->] (C11) -- (C22);
\draw[->] (C11) -- (C32);

\end{tikzpicture}
\caption{Example of a process-time graph $PT^2$ at time $t=2$ with $n=3$ processes and initial values $x=(1,0,1)$.
Process~$1$'s view $V_{\{1\}}(PT^2)$ is highlighted in bold green.}
\label{fig:pt}
\end{figure}

Let $\PT^t$ be the set of all possible
process-time graphs at time~$t\geq 0$, which is finite for any $t\geq 0$.
Furthermore, let
$\PTomega = \PTzero \times \PTone \times \dots$ be the set of all infinite sequences of possible process-time graphs.\footnote{Please note that we slightly 
abuse the notation $\PTomega$ here, which normally represents 
$\PT \times\PT\times \dots$.}

Given an input domain~$\VI$,
every message adversary uniquely corresponds to a subset~$PS$ of~$\PTomega$
generated by the graph sequences admissible under the message adversary.

Note that process-time graphs are \emph{independent} of the particular algorithm used, but
do depend on the input values.
For conciseness, we will use the term process-time graphs for the elements
of $\PTomega$ as well.
We will denote elements of $\PTomega$ by Roman letters $a,b,\dots$
(or sometimes $PT,PT',\dots$).



%US: Vielleich bei irgend einer Application nützlich?
%
%For message passing systems, 
%the events $E_p^{t.5}$ happening at process $p$ can be the following:
%\begin{enumerate}
%\item[(i)] $E_p^{t.5}=\emptyset$ (stuttering step), in which case $C_p^{t+1}=C_p^t$, 
%\item[(ii)] $E_p^{t.5}=2^{M_p^t}\setminus\emptyset$ (pure receive step), 
%where $M_p^{t.5} \in \M_p$ denotes the set of messages sent to $p$ in the computing steps 
%up to and including time $t.5$; $\M_p$ denotes the set of all possible messages 
%sent to $p$. It generates the set $R_p^{t.5} \subseteq \M_p$ of messages 
%received by but not processed by $p$ up to and including time $t.5$.
%\item[(iii)] $E_p^{t.5}=\{\go} \cup 2^{M_p^t}$ (receive and processing step),
%which first generates $R_p^{t.5}$ as in (ii) and then applies $p$'s \emph{local transition
%function} $\tau_p: \C_p \times \M_p \to \C_p$ that represents $p$'s instance of $\A$, 
%which computes the successor configuration
%$C_p^{t+1}=\tau_p(C_p^t,R_p^{t.5})$, based on the current configuration $C_p^t$ and
%the set of received but not yet processed messages $R_p^{t.5}$.
%\item[(iv)] $E_p^{t.5}=\{\crash} \cup 2^{M_p^t}$ (crash step), in which case 
%all received messages are discarded and $C_p^{t+1}=\bot$. Note that crashes are
%persistent, i.e., only crash steps may occur after the very first one.
%\end{enumerate}



\subsection{Bivalence-based Impossibilities}
\label{sec:bivalence}

Our topological results shed some new light on the now standard technique of
bivalence-based impossibility proofs introduced in the celebrated FLP paper \cite{FLP85},
which have been generalized in \cite{MR02} and used in many different contexts: Our
results reveal that the forever bivalent executions constructed inductively in 
bivalence proofs such as \cite{SW89,SWK09} and \cite{BRSSW18:TCS,WSS19:DC}
are just the common limit of two infinite sequence of executions $\alpha_0,\alpha_1,\dots$
all contained in, say, $\Gamma(0)$ and  $\beta_0,\beta_1,\dots$ all contained in $\Gamma(1)$ that
have a common limit $\alpha_k\to\hat{\alpha}$ and  $\beta_k\to\hat{\beta}$
in some $\{p\}$-view topology with $d_{\{p\}}(\hat{\alpha},\hat{\beta})=0$.

More specifically, what is common to these proofs is that one shows that, for any
consensus algorithm, there is an admissible forever bivalent run. This is usually done inductively,
by showing that there is a bivalent initial configuration and that, given a bivalent
configuration $C^{t-1}$ at the end of round $t-1$, there is a 1-round extension
leading to a bivalent configuration $C^t$ at the end of round $t$.
By definition, bivalence of $C^t$ means that there are two admissible executions $\alpha_t$ with 
decision value 0 and $\beta_t$ with decision value 1 starting out from $C^t$, i.e.,
having a common prefix that leads to $C^t$. Consequently, their distance, in any $\{p\}$-view topology, satisfies $d_{\{p\}}(\alpha_t,\beta_t) < 2^{-t}$. Note that this 
is also true for the more general concept of a bipotent configuration $C^t$, as
introduced in \cite{MR02}.

By construction, the $(t-1)$-prefix of $\alpha_t$ and $\alpha_{t-1}$ are the same, for
all $t$, which implies that they converge to a limit $\hat{\alpha}$ (and analogously for $\hat{\beta}$), see Figure~\ref{fig:noncompactMA} for an illustration. 
Therefore, these executions match Definition~\ref{def:fairunfair}, and Corollary~\ref{cor:consensusimpfair} implies that the stipulated consensus algorithm cannot be correct.
Concrete examples are the lossy link impossibility \cite{SW89}, i.e., the impossibility of consensus under an oblivious
message adversary for $n=2$ that may choose any graph out of the set $\{\leftarrow,\leftrightarrow,\rightarrow\}$, and the impossibility of solving consensus with vertex-stable source components with insufficient stability interval \cite{BRSSW18:TCS,WSS19:DC}. 
In the case of the oblivious
lossy link message adversary using the reduced set $\{\leftarrow,\rightarrow\}$ considered
in \cite{CGP15}, consensus is solvable and there is no forever bivalent run.
Indeed, there exists a consensus algorithm, such that all configurations reached after the first round are already univalent.



\subsection{Compact Message Adversaries}
\label{sec:closed}

In this section, we consider message adversaries (like oblivious ones \cite{SW89,CGP15}) that are limit-closed, in the sense
that every convergent sequence of process-time graphs 
$a_0,a_1,\dots$ with $a_i \in PS$ for every $i$ has a limit $\hat{a} \in PS$. An illustration is shown in Fig.~\ref{fig:compactMA},
where the blue dots represent the $a_i$'s and $\times$ the limit point $\hat{a}$ at the boundary.


\tikzset{cross/.style={cross out, draw=black, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt},
cross/.default={1pt}}

\begin{figure}[ht]
\centering  
 \begin{tikzpicture}[scale=0.3]
\def\firstcircle{(0,0) ellipse (3cm and 2cm )}
\def\secondcircle{(0,5) ellipse (3.5cm and 2.5cm)}
\def\thirdcircle{(6,0) ellipse (2.5cm and 1.5cm)}
\def\fourthcircle{(6,3.8) ellipse (2cm and 1.5cm)}
\draw[blue!50!cyan, ultra thick] \firstcircle node[text=black] {$PS_{z_0}$};
    \draw[blue!50!cyan, ultra thick] \secondcircle node[text=black]  {$PS_{z_0'}$};
    \draw[green!50!cyan, ultra thick] \thirdcircle node[text=black]  {$PS_{z_1}$};
   \draw[green!50!cyan, ultra thick] \fourthcircle node[text=black]  {$PS_{z_1'}$};
\begin{scope}[rotate=-20]
\foreach \i in {0,...,5} {
  \draw[fill,color=blue] ({2.2-2*1.3^(-\i)},5.5) circle (0.1);
}
\draw ({2.2-2*1.3^(-5)},5.5) node[cross=4pt,blue, thick]{};
\end{scope}
\end{tikzpicture}%
\caption{Examples of two connected components of the decision sets $PS(0)=PS_{z_0}\cup PS_{z_0'}$ and
 $PS(1)=PS_{z_1}\cup PS_{z_1'}$ for a compact message adversary. They are closed in $\PTomega$, hence 
contain all their limit points (marked by $\times$) and have a distance $>0$ by Theorem~\ref{thm:compactsetdistance}.}\label{fig:compactMA}
\end{figure}

In this case, the set of admissible process-time graph sequences $PS$ is closed and hence
a compact subspace both in any $P$-view topology and in the minimum topology. 
Moreover, we obtain:

\begin{corollaryrep}[Decision sets for compact MAs are compact]\label{cor:closeddecsetscompact}
For every correct consensus algorithm for a compact message adversary and every $v\in\VO$, $PS(v)$ is closed in $PS$ and compact, and $d_{\{p\}}(PS(v),PS(w))>0$ for any $v,w\neq v \in
\VO$ and $p\in[n]$, and hence also $d_{\min}(PS(v),PS(w))>0$. 

Moreover, there are only finitely many different
connected components $PS_{x}$, $x\in PS$, which are all compact, and for every $x,y$ with $PS_x\neq PS_y$, it holds that $d_{\{p\}}(PS_x,PS_y)>0$ and hence also $d_{\min}(PS_x,PS_y)>0$.
\end{corollaryrep}
\begin{proof}
Since all decision sets $PS(v)$ are closed in $PS$ by Theorem~\ref{thm:char} and $PS$
is compact for a compact message adversary, it follows that every $PS(v)$ is also compact. From Theorem~\ref{thm:compactsetdistance} it hence follows that $d_{\{p\}}(PS(v),PS(w))>0$. As this holds for every $p\in[n]$, we also have $d_{\min}(PS(v),PS(w))>0$.

Since every connected component $PS_x$ of $PS$ that contains $x$ is closed in $PS$, as the closure of a connected subspace is also connected by \cite[Lemma~23.4]{Munkres} and a connected component is maximal, the same arguments 
as above also apply to $PS_x$. To show that there are only finitely many different $PS_{z_v}$ for $v$-valent sequences $z_v\in PS$, observe that $PS(v)=\bigcup_{z_v \in PS} PS_{z_v}$ is an open covering of $PS(v)$. Since the latter is compact,
there is a finite sub-covering $PS(v)=PS_{z_v^1} \cup \dots \cup PS_{z_v^m}$, and
all other $PS_{z_v}$ for a $v$-valent $z_v$ must be equal to one of those,
as connected components are either disjoint or identical.
\end{proof}

We now make the abstract characterization of Theorem~\ref{thm:char} and our meta-procedure
more operational, by introducing the $\varepsilon$-approximation of the connected
component $PS_z$ that contains a process-time graph $z \in PS$, typically for some $\varepsilon = 2^{-t}$, 
$t\geq 0$. It is constructed iteratively, using finitely many iterations (since the number of different possible
$t$-prefixes satisfies $|\PT^t|<\infty$) of the following algorithm:

\begin{definition}[$\varepsilon$-approximations]\label{def:epsilonPSv}
Let $z\in PS$ be an admissible process-time graph. In the minimum topology, 
we iteratively define $PS_{z}^\varepsilon$, for $\varepsilon>0$, as follows:
$PS_{z}^\varepsilon[0]=\{z\}$; for 
$\ell>0$, $PS_{z}^\varepsilon[\ell] = \bigcup_{a \in PS_{z}^\varepsilon[\ell-1]}(B_{\varepsilon}(a) \cap PS)$; and $PS_{z}^\varepsilon=PS_{z}^\varepsilon[m]$ where $m<\infty$ is such
that $PS_{z}^\varepsilon[m]=PS_{z}^\varepsilon[m+1]$. For $v\in\VO$, the $\varepsilon$-approximation $PS^\varepsilon(v)$ is defined as $PS^\varepsilon(v)=\bigcup_{z_v \in PS}PS_{z_v}^\varepsilon$, where
every $z_v$ denotes a $v$-valent process-time graph.
\end{definition}

\begin{lemmarep}[Properties of $\varepsilon$-approximation]\label{lem:propertiesapproxclosed}
For every $\varepsilon>0$, every $v,w\in\VO$, every $z\in PS$, $v$-valent $z_v$, and every $w$-valent $z_w$, the $\varepsilon$-approximations have the
following properties:
\begin{enumerate}
\item[(i)] For a compact message adversary, there are only finitely many different $PS_{z}^\varepsilon$, $z\in PS$. 
\item[(ii)] For every $0<\varepsilon'\leq\varepsilon$, it holds that 
$PS_{z_v}^{\varepsilon'} \subseteq PS_{z_v}^\varepsilon$.
\item[(iii)] $PS_{z_v}^\varepsilon \cap PS_{z_w}^\varepsilon\neq \emptyset$ implies $PS_{z_v}^\varepsilon = PS_{z_w}^\varepsilon$.% for every $v,w\in \VO$. 
\item[(iv)] $PS_{z} \subseteq PS_{z}^\varepsilon$.
\end{enumerate}
\end{lemmarep}
\begin{proof}
Properties (ii)--(iv) hold for arbitrary message adversaries:
To prove (ii), it suffices to mention $B_{\varepsilon'}(a) \subseteq B_{\varepsilon}(a)$.
As for (iii), if $a \in PS_{x}^\varepsilon \cap PS_{y}^\varepsilon\neq 0$, the iterative construction of $PS_{x}^\varepsilon$ would reach $a$, which would cause it
to also include the whole $PS_{y}^\varepsilon$, as the latter also reaches $a$. If (iv) would not hold,
$PS_{z}$ could be separated into disjoint open sets, which contradicts connectivity.
Finally, (i) holds for compact message adversaries, since Corollary~\ref{cor:closeddecsetscompact}  implies that there are only finitely many
 different connected components $PS_{z}$, which carry over to $PS_{z}^\varepsilon$ by (iii) and (iv).
\end{proof}

We now show that  $PS_{x}^\varepsilon$ and $PS_{y}^\varepsilon$ for sequences $x$ and $y$ with $PS_x \neq PS_y$ have a distance $>0$, provided $\varepsilon$ is sufficiently small:

\begin{lemmarep}[Separation of $\varepsilon$-approximations for compact MAs]\label{lem:closedepsilonapprox}
For a compact message adversary that allows to solve consensus, let $x\in PS$ and $y\in PS$ be such that $PS_x \neq PS_y$. Then, there is some 
$\epsilon>0$ such that, for any $0<\varepsilon'\leq \varepsilon$, it holds that 
$d_{\min}(PS_{x}^{\varepsilon'}, PS_{y}^{\varepsilon'})>0$. 
\end{lemmarep}
\begin{proof}
According to Corollary~\ref{cor:closeddecsetscompact}, the components $PS_x$ and $PS_y$ are compact.
Theorem~\ref{thm:compactsetdistance} reveals that we have $d_{\min}(PS_x,PS_y)=d > 0$. 
By Lemma~\ref{lem:propertiesapproxclosed}.(iv), for every $\varepsilon>0$,
$PS_{x} \subseteq PS_{x}^\varepsilon$ and $PS_{y} \subseteq PS_{y}^\varepsilon$. 
Therefore, setting $\varepsilon< d/2$ secures $d_{\min}(PS_{x}^{\varepsilon},PS_{y}^{\varepsilon}) > 0$. 
\end{proof}

We immediately get the following corollary, which allows us to reformulate Theorem~\ref{thm:charbroadcastability}
as given in Theorem~\ref{thm:closedsufficiency}.

\begin{corollary}[Matching $\varepsilon$-approximation]\label{cor:matchingapproximationclosed}
For a compact message adversary, if $\varepsilon>0$ is chosen in accordance with Lemma~\ref{lem:closedepsilonapprox},
then $PS_z^\varepsilon = PS_z$  for every $z\in PS$.
\end{corollary}

\begin{theoremrep}[Consensus characterization for compact MAs]\label{thm:closedsufficiency}
A compact message adversary allows to solve consensus if and only if there is some 
$\varepsilon>0$ such that every $v$-valent $PS_{z_v}^{\varepsilon}$, $v\in \VO$, is broadcastable for some process. 
\end{theoremrep}
\begin{proof}
Our theorem follows from Theorem~\ref{thm:charbroadcastability} in conjunction with Corollary~\ref{cor:matchingapproximationclosed}.
\end{proof}
Note carefully that if consensus is solvable, then, for every $0<\varepsilon'\leq \varepsilon$, the universal algorithm
from Theorem~\ref{thm:char} with $PS(v)=PS^{\varepsilon'}(v) \cup PS\setminus\bigcup_{w\neq v\in\VO}PS^{\varepsilon'}(w)$ for some arbitrary value $v\in\VO$, and $PS(w)=PS^{\varepsilon'}(w)$ for the remaining $w\in\VO$, can be used.

We conclude this section with noting that checking the broadcastability of  $PS_{z_v}^{\varepsilon}$ can be done by checking
broadcastability only in \emph{finite} prefixes. More specifically, like the decision function $\Delta$ of consensus, the function $T(a)$ that gives the round by which every process in $a\in PS$ has $(p,0,x_p(a))$ of the broadcaster $p$ in its view is locally constant for a sufficiently small neighborhood, namely,  $B_{2^{-T(a)}}(a)$, and is hence continuous in the $\max$-topology and hence in any of
our topologies. Since $PS_{z_v}=PS_{z_v}^\varepsilon$ is compact, $T(a)$ is in fact uniformly continuous and hence attains its maximum $\hat{T}$ in $PS_{z_v}^\varepsilon$. It hence suffices to
check broadcastability in the $t$-prefixes of $PS_{z_v}^{\varepsilon}$ for $t=\max\{\lfloor \log_2(1/\varepsilon)\rfloor,\hat{T}\}$
in Theorem~\ref{thm:closedsufficiency}.

\subsection{Non-compact Message Adversaries}
\label{sec:nonclosed}

In this section, we finally consider message adversaries that are not limit-closed, like the ones of  \cite{FG11,Pfl18:master,WSS19:DC}. 
Unfortunately, we cannot use the $\varepsilon$-approximations
according to Definition~\ref{def:epsilonPSv} for non-compact message adversaries. Even if $\varepsilon$ is made arbitrarily 
small, Lemma~\ref{lem:closedepsilonapprox} does not hold. An illustration is shown in Fig.~\ref{fig:noncompactMA}. Hence, adding a ball $B_{\varepsilon}(a)$ in the iterative construction of $PS_{z}^\varepsilon$, where $d_{\min}(a,r)<\epsilon$ for some forbidden limit sequence $r$, inevitably lets the construction grow into some  $PS_{z'}^\varepsilon$ where $z'$ has a different valence than $z$. Whereas this could be avoided by adapting $\varepsilon$ when coming close to $r$, the resulting approximation does not provide any advantage over directly using the connected components.

\begin{figure}[ht]
\centering  
 \begin{tikzpicture}[scale=0.8]
\pgfmathsetseed{2}
  \draw [blue!50!cyan, dashed, ultra thick, shift={(0,0)}] 
    plot [smooth cycle, tension=1, domain=0:320, samples=18] (\x:{4/3+rand/3}) 
        node[left=0cm,above=0.2cm,text=black] {$PS_{z_{0}}\qquad$} ;
  \draw [green!50!cyan, dashed, ultra thick, shift={(3.1,0)}] 
    plot [smooth cycle, tension=1, domain=0:320, samples=18] (\x:{4/3+rand/3}) 
        node[left=0cm,above=0.2cm,text=black] {$PS_{z_{1}}\qquad$} ;
  \draw [blue!50!cyan, dashed, ultra thick, shift={(0,3.1)}] 
    plot [smooth cycle, tension=1, domain=0:320, samples=18] (\x:{4/3+rand/3}) 
        node[left=0cm,above=0.2cm,text=black] {$PS_{z_{0}'}\qquad$} ;
 \draw [green!50!cyan, dashed, ultra thick, shift={(3.1,3.1)}] 
    plot [smooth cycle, tension=1, domain=0:320, samples=18] (\x:{4/3+rand/3}) 
        node[left=0cm,above=0.2cm,text=black] {$PS_{z_{1}'}\qquad$} ;
\foreach \i in {0,...,5} {
  \draw[fill,color=green!80!black] ({1.39+1.5^(-\i)},0.3) circle (0.05);
  \draw[fill,color=blue] ({1.39+1.5^(-5)-1.5^(-\i)},0.3) circle (0.05);
}
\draw ({1.36+1.5^(-5)},0.3) node[cross=4pt,red, thick]{};
\end{tikzpicture}%
\caption{Examples of two connected components of the decision sets $PS(0)=PS_{z_0}\cup PS_{z_0'}$ and
 $PS(1)=PS_{z_1}\cup PS_{z_1'}$ for a non-compact message adversary. They are not closed in $\PTomega$ and may have
distance 0; common limit points (like for $PS_{z_0}$ and $PS_{z_1}$, marked by $\times$) must hence be excluded by
Corollary~\ref{cor:consensusseparation}.}
\label{fig:noncompactMA}
\end{figure}



Actually, this is in accordance with the existing solutions 
for non-compact message adversaries we are aware of, albeit they typically use their complement, namely, excluded sequences.
For example, the binary consensus algorithms for $n=2$ given in \cite{FG11,Pfl18:master} assume that the algorithm 
knows a fair or a pair of  unfair sequences a priori, which effectively partition the sequence space into two connected 
components.\footnote{Note that there are uncountably many choices for separating $PS(0)$ and $PS(1)$ here.} 
The $(D+1)$-VSRC message adversary of \cite{WSS19:DC} even excludes all 
sequences without a root component that is vertex-stable for at least $D+1$ rounds, where $D$ is the dynamic diameter 
that ensures broadcastability by all root members, which renders the remaining connected components broadcastable.

We restate the following necessary and sufficient condition for solving consensus with a non-compact message adversary
from Theorem~\ref{thm:charbroadcastability}:

\begin{theorem}[Consensus characterization for non-compact MAs]\label{thm:nonclosedsufficiency}
A non-compact message adversary allows to solve consensus if and only if every $v$-valent 
$PS_{z_v}$, $v\in \VO$, is broadcastable for some process. 
\end{theorem}

We will finally prove that the set of to be excluded limit 
sequences for any decision set $PS(v)$ is compact for a message adversary
that allows to solve consensus:

\begin{lemmarep}[Compactness of excluded sequences]\label{def:compactnessforbidden}
Let $PS(v)$, $v\in\VO$, be any decision set of a correct consensus algorithm for an arbitrary message
adversary,   $\cl{PS}(v)$ be its closure in $\PTomega$ and $\inte{PS}(v)$ its interior. 
Then, $\bd{PS}(v)=\cl{PS}(v) - \inte{PS}(v)$, which is the set of to be excluded limit points, is compact.
\end{lemmarep}
\begin{proof}
The closure $\cl{PS}(v)$ is closed by definition.
Since the complement of the interior $\inte{PS}(v)^C$ is also closed by definition,
it follows that $\bd{PS}(v)=\cl{PS}(v) - \inte{PS}(v) = \cl{PS}(v) \cap \inte{PS}(v)^C$ is also closed. 
As a closed subset of the compact set $\cl{PS}(v)$, $\bd{PS}(v)$ is hence compact. 
\end{proof}

\section{Conclusions}
\label{sec:conclusions}

We provided a complete topological characterization of the solvability of consensus
in synchronous directed dynamic networks of arbitrary size controlled by a general
message adversary: Consensus can only be solved when the space of admissible process-time
graph sequences can be partitioned into at least two non-empty sets that are both
closed and open in specific topologies. This requires exclusion of certain fair and unfair
limit sequences, which limit broadcastability and 
happen to coincide with the forever bivalent executions constructed
in bivalence and bipotence proofs.

Part of our future work will be devoted to a generalization of our topological framework to other 
distributed computing models and, most importantly, to other decision problems.
Another very interesting area of future research is to study the homology
of non-compact message adversaries, i.e., the topological structure of the
space of admissible executions using combinatorial topology.

